RoboNet: Large-Scale Multi-Robot Learning

Robot learning has emerged as a promising tool for taming the complexity and diversity of the real world. Methods based on high-capacity models, such as deep networks, hold the promise of providing effective generalization to a wide range of open-world environments. However, these same methods typically require large amounts of diverse training data to generalize effectively. In contrast, most robotic learning experiments are small-scale, single-domain, and single-robot. This leads to a frequent tension in robotic learning: how can we learn generalizable robotic controllers without having to collect impractically large amounts of data for each separate experiment? In this paper, we propose RoboNet, an open database for sharing robotic experience, which provides an initial pool of 15 million video frames, from 7 different robot platforms, and study how it can be used to learn generalizable models for vision-based robotic manipulation. We combine the dataset with two different learning algorithms: visual foresight, which uses forward video prediction models, and supervised inverse models. Our experiments test the learned algorithms' ability to work across new objects, new tasks, new scenes, new camera viewpoints, new grippers, or even entirely new robots. In our final experiment, we find that by pre-training on RoboNet and fine-tuning on data from a held-out Franka or Kuka robot, we can exceed the performance of a robot-specific training approach that uses 4x-20x more data. For videos and data, see the project webpage: https://www.robonet.wiki/

==> experimental_eval.tex <==


\section{Experimental Evaluation}
%%SL.6.30: It's particularly important in this paper to provide a thorough discussion of what our experiments actually aim to study -- pay extra attention to this!

%%CF: I added this:
The core goal of our experimental evaluation is to study the viability of large-scale data-driven robot learning as a means to acquire broad generalization.
To that end, we design our experiments to study the following questions: (1) can we leverage RoboNet to enable zero-shot generalization or few-shot adaptation to novel viewpoints, novel grippers, and novel robotic platforms? (2) how does the breadth and quantity of data affect generalization?, (3) do predictive models trained on RoboNet memorize individual contexts or learn generalizable concepts that are shared
across contexts, and (4) does our proposed accuracy metric correlate with planning performance on the real robot?

%%CF.7.4: TODO - if we use the context model, we should also have a question about that.

% \subsection{Manipulation Benchmarks}  %FE: don't need a section here!
%%SL.6.30: Discuss the tasks on which we evaluate (e.g., pushing/lifting/whatever), with pictures

We evaluate our method and the benefits of training on the data in RoboNet by analyzing the performance of the planner on a set of common, every-day-life manipulation tasks. 

We show both qualitative experiments and quantitative evaluations. For measuring the quantitative performance in an object-relocation task we hand-annotate the positions of the objects after executing the actions computed by the planner and measure the euclidean distance to the corresponding goal position.

% \subsection{Training Robot-Agnostic Visual Predictive Models}
%%FE: We can merge this with "Generalization Experiments" SL.6.30: This is for video prediction results and qualitative results



\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{placeholder.png}
    \caption{\small{Saturation Analysis, Bar graph}}
    \label{fig:sat_analysis}
\end{figure}
\subsection{Generalization Experiments}


% \begin{tabular}{|c|c|c|c|c|c|}
% \toprule
% {} &  \multicolumn{2}{c}{Zero-Shot} & \multicolumn{3}{c}{Fine-Tuning}\\
% \midrule
% Experiment   &  Gen. to new view-point & Gen. to new gripper & Cross-domain transfer  & Gen. to new robot & Gen. to new robot\\ 
% \hline
% Training Data   &  All of RoboNet & All of RoboNet   & \makecell{Hard objects: Sawyer, Baxter, Franka\\ Soft objects: Sawyer}  & All of RobotNet except Baxter & All
% of RoboNet except WidowX \\
% \hline
% Test Data   &  Sawyer with unseen view-poitns &  Sawyer wtih unseen gripper   & Soft objects on Baxter  & Baxter data & WidowX data\\
% \bottomrule
% \end{tabular}
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/experiment_overview.pdf}
    \caption{\small{Overview of generalization experiments}}
    \label{fig:sat_analysis}
\end{figure}


%%SL.6.30: This is the main experimental results section, with \paragraph headings for generalization to viewpoint, gripper, and eventually to full robot
We study how the diversity in the training dataset affects the models' capability to generalize in a variety of different ways. To this end we need to distinguish between \emph{zero-shot generalization}, where no additional data from the target domain is available and \emph{adaptation}, where the networks are fine-tuned on a relatively small amount of data from the target domain. 

\textbf{Viewpoint generalization}
Viewpoint generalization is one of the simpler forms of generalization, since changing the viewpoint only transforms the observations, it does not affect the underlying physics in the environment. We compare a model that has been trained on ?? different viewpoints with a model that was only trained on single viewpoint. Table ?? shows that a model trained on a variety of viewpoints significantly outperforms a model that was only trained on a single viewpoint.

\textbf{Cross-Domain Object Transfer}
We find that the models learn shared generalizable concepts by observing that certain types of physical interactions learned with one robot interacting with a particular kind of object transfer to another robot which has not interacted with this kind of object. 
In particular we tested whether training on data from three different robots, a Franka, a Sawyer and a Baxter robot, where cloth was only present in the trajectories with the Sawyer robot, would allow the model to make accurate predictions for cloths on a Baxter robot.

% We observed that zero-shot generalization does not work in this case, which might have been caused by the fact that the Baxter robot we evaluate on is in a different lab setting than where the Baxter data was collected.

When fine-tuning the model on 300 trajectories from the Baxter interacting with cloth, we indeed observe accurate predictions. We further test control and find that the Baxter is successful in manipulating cloth in ?? out of ?? trials. By contrast when pre-training on data only from Sawyers we only get ?? out of ?? successes and when training on 300 trajectories from scratch, i.e. random initialization we obtain only ?? successes. This indicates that more diversity in the data helps transfer learning, and allows effectively pooling robotic experience.

\textbf{Zero-Shot Generalization to new Gripper}
The capability to instantly generalize to different gripper can be of large practical value since it eliminates a potentially time-consuming data collection and adaptation. Here we show that a model trained on the entirety of RoboNet zero-shot generalizes to a different gripper, not contanined in the training set. Concretely we replaced the gripper on the Sawyer robots with a Robotiq gripper, that was not part of the training set. We compare zero-shot generalization performance on rigid object relocation tasks for a model trained on all of RoboNet with a model only trained on data from Sawyer robots. The benchmark results clearly indicate that more diversity in the training set helps zero-shot performance.

\textbf{Adaptation to new Robot}
Generalizing to a robot that was not part of the training set is perhaps the most challenging form of generalization we are testing in this work. A different robot platform implies not only different appearance but also different object interaction dynamics, kinematics and workspace boundaries. Because of all these factors generalizing in without any additional data is currently beyond reach. Instead we evaluate the performance after finetuning on new data from the target platform.

We perform two different experiments: Training on all of RoboNet except the Baxter robot and finetuning on 600 additional trajectories from said robot. The second experiment is the same, except holding out the WidowX robot. 
We compare the performance of these models in control trials with the performance of models that only pretrained on a single robot, in this case the Sawyer roobt.

Again we observe that models pretrained on more diverse data performed significantly better than model trained only the same amount, but less diverse data.


\subsection{Validating the Pixel-Motion Accuracy Metric}
%%SL.6.30: This is to show correlation between metrics and real-world performance
\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{placeholder.png}
    \caption{\small{Accuracy metric correlation experiments}}
    \label{fig:accuracy_metric}
\end{figure}

We conduct experiments that show that our proposed accuracy metric for video-prediction outlined in \autoref{subsec:cross_domain} correlates better with performance in robot control experiments than common video-prediction metrics such as MSE, SSIM, PSNR.
We hypothesize that this is because our proposed metric evaluates the accuracy of motion predictions rather than accurate predictions of absolute RGB values. MSE, SSIM, PSNR are very sensitive to small displacements of objects or arm positions, while they are insensitive or in some cases invariant for large object position differences, in particular when there is no overlap between the pixels of an object in the predict image and ground-truth image.

\subsection{Data Saturation Analysis}
How many trajectories are necessary for training until a model saturates in validation performance? Knowing this number, and what influences it, is important since it determines the required minimum effort for data collection. We found that this number mainly depends on two factors, the model capacity and the diversity of the training data.

For a dataset with a single robot and multiple view-points we found that a video-prediction model with XX parameters saturated at around 4.500 trajectories.
For multiple robots and multiple viewpoints the saturation point was at ?? trajectories, total over all robots. See \autoref{fig:sat_analysis} for an overview.
When training on data from 6 robots the saturation point was at ?? trajectories. 

These results indicate that our models heavily underfit and \emph{bigger models} would be beneficial to obtain higher accuracy and allow training on a greater number of domains.

==> robot_agnostic_control.tex <==
\section{Robot-Agnostic Visual Control}
%%SL.6.30: This section focuses on the robot-agnostic control method, not the dataset. The purpose of this section is to articulate the main technical point that we can build a single model that can control multiple robots. This is where we talk about embedding and finetuning. In the opener, discuss and motivate having one model control different robots, and the benefits of doing this (e.g., can control a new robot without even having collected any data from it), and discuss how there are three ways: 0-shot, embedding, and finetuning

The ability for a robotic planner to generalize in zero shots means that for a new target domain no additional data is required. This is highly desirable since a system can then be deployed to the target domain with very little effort, an important step for allowing wider applicability of robotic manipulation. Furthermore if a \emph{single model} can be used for many tasks and environments, the practical value is also much higher than if separate models had to be selected, e.g. by a human operator.
We show that by training a single model on the data in RoboNet we can achieve zero-shot generalization to new domains, even when they have significant differences to training domains. 

When the differences to the training domains become too large and zero-shot generalization is not possible anymore, we can still adapt a model trained on the entirety of the data to the target domain at hand.

\subsection{Zero-Shot Generalization to New Robots}

While zero-shot generalization is the most preferable form of generalization, it only works if the target domain is close enough to the training data. This should mean that the broader and more diverse the training data distribution is, the more likely it is to generalize in zero-shots. To prove this hypothesis we compare the performance of our algorithm when trained on the entirety of the data collected from 6 different robot arms with the performance obtained when only trained on the data from one robot arm. Since we are only interested in studying the effects of \emph{data diversity} we make sure that the numbers of training data points are the same in both cases.


\subsection{Cross-Domain Generalization}
\label{subsec:cross_domain}
If experience collected with a particular robot in a particular environment transfers to another robot in a different environment, then this means that combining the experience from many robots allows creating a system with the effective experience of all robots combined. 

In this work we test whether experience from interacting with a particular object class and a particular robot transfers to different robot from which we haven't collected any data of this class. Concretely train on the complete RoboNet database which contains \emph{soft-objects}, i.e. towels and clothes only in combination with a Sawyer robot. Whether the capability to correctly predict the dynamics of soft objects and the capability of manipulating soft object transfers to a different robot, in this case a Baxter robot. Note that RoboNet contains signicant numbers of trajectories with Baxter data interacting with \emph{hard objects}.

%\subsection{Learning Dynamic Robot Identification via Domain Embeddings}
%%SL.6.30: the embedding model

\subsection{Rapid Finetuning to New Robots and Domains}
%%SL.6.30: talk about finetuning, be sure to motivate that this is to get good performance even when 0-shot and embeddings are not enough i.e. because the shift is too large

When the difference between the training domains and the target domain is large, for example when the target domain uses a different robot platform, we can fine-tune a model pretrained on the RoboNet database to adapt to the target domain. 

Here we again analyze the effects of diversity in the database used for pre-training. 








